Investigating episodic mass loss in evolved massive stars: I. Spectroscopy of dusty massive stars in ten southern galaxies

The ASSESS project aims to determine the role of episodic mass-loss in the evolution of massive stars. As a first step, we construct a catalog of spectroscopically identified dusty, evolved massive stars in ten southern galaxies for which Spitzer point-source catalogs are available. We conducted multi-object spectroscopy of dusty massive star candidates in these galaxies (spanning Z = 0.06-1.6 Zo) using the VLT. We obtained 763 spectra in WLM, NGC 55, NGC 247, NGC 253, NGC 300, NGC 1313, NGC 3109, Sextans A, M83 and NGC 7793. The targets were selected using their Spitzer photometry, by prioritizing targets with a strong infrared excess. We determined a spectral classification for each target. Additionally, we used archival images from the HST to provide a visual classification for 80 targets, as a star, cluster, or galaxy. We provide a catalog of 541 spectroscopically classified sources including 185 massive stars, of which 154 are newly classified massive stars. The catalog contains 129 red supergiants, 27 blue supergiants, 10 yellow supergiants, four luminous blue variable candidates, seven supergiant B[e] stars and eight emission line objects. Evidence for circumstellar dust is found in 24% of these massive stars, based on their infrared colors. We report a success rate of 28% for identifying massive stars among our observed spectra, while the average success rate of our priority system in selecting evolved massive stars was 36%. Additionally, the catalog contains 21 background galaxies (including AGN and quasars), 10 carbon stars and 99 HII regions. We measured the line ratios [NII]/Ha and [SII]/Ha for 76 HII regions and 36 other spectra with nebular emission-lines, thereby identifying eight sources with shocked emission. We present the largest catalog of evolved massive stars and in particular of red supergiants in nearby galaxies at low Z beyond the Local Group.

==> Figure_AllSlitLocations.tex <==


\clearpage

\subsection{M83 Field B}

\vfill
\begin{figure*}[h!]
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_M83_FieldB.pdf}}
  	\caption{Mask layout for M83 Field B.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldB_Slits/M83_FieldB_Slit35.pdf}& 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for M83 Field B.}
\end{figure}




\clearpage

\subsection{M83 Field C}

\vfill
\begin{figure*}[h!]
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_M83_FieldC.pdf}}
  	\caption{Mask layout for M83 Field C.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/M83_FieldC_Slits/M83_FieldC_Slit34.pdf}\\ 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for M83 Field C.}
\end{figure}




\clearpage

\subsection{NGC55 Field A}

\vfill
\begin{figure*}[h!]
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_NGC55_FieldA.pdf}}
  	\caption{Mask layout for NGC55 Field A.}
\end{figure*}
\vfill

%\clearpage

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit53.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit54.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit55.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit56.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit57.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit58.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit59.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit60.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit61.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit62.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit63.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit64.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldA_Slits/NGC55_FieldA_Slit65.pdf}& 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for NGC55 Field A.}
\end{figure}




\clearpage
\subsection{NGC55 Field B}
\vfill
\begin{figure*}[h!]
	\center
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_NGC55_FieldB.pdf}}
  	\caption{Mask layout for NGC55 Field B.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit53.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit54.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit55.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit56.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit57.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit58.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit59.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldB_Slits/NGC55_FieldB_Slit60.pdf}&
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for NGC55 Field B.}
\end{figure}


\clearpage
\subsection{NGC55 Field C}
\vfill
\begin{figure*}[h!]
	\center
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_NGC55_FieldC.pdf}}
  	\caption{Mask layout for NGC55 Field C.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit53.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit54.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit55.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit56.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit57.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit58.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit59.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit60.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit61.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit62.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit63.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit64.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC55_FieldC_Slits/NGC55_FieldC_Slit65.pdf}& 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for NGC55 Field C.}
\end{figure}

\clearpage
\subsection{NGC247 Field A}
\vfill
\begin{figure*}[h!]
	\center
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_NGC247_FieldA.pdf}}
  	\caption{Mask layout for NGC247 Field A.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit53.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit54.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit55.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit56.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit57.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit58.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit59.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit60.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit61.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit62.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit63.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit64.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit65.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit66.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit67.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit68.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit69.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit70.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldA_Slits/NGC247_FieldA_Slit71.pdf}& 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for NGC247 Field A.}
\end{figure}

\clearpage
\subsection{NGC247 Field B}
\vfill
\begin{figure*}[h!]
	\center
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_NGC247_FieldB.pdf}}
  	\caption{Mask layout for NGC247 Field B.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit53.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit54.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit55.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit56.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit57.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit58.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit59.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit60.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit61.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit62.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit63.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit64.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit65.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit66.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit67.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit68.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit69.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC247_FieldB_Slits/NGC247_FieldB_Slit70.pdf}\\ 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for NGC247 Field B.}
\end{figure}


\clearpage
\subsection{NGC253 Field A}
\vfill
\begin{figure*}[h!]
	\center
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_NGC253_FieldA.pdf}}
  	\caption{Mask layout for NGC253 Field A.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit53.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit54.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit55.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit56.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit57.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldA_Slits/NGC253_FieldA_Slit58.pdf}\\ 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for NGC253 Field A.}
\end{figure}


\clearpage
\subsection{NGC253 Field B}
\vfill
\begin{figure*}[h!]
	\center
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_NGC253_FieldB.pdf}}
  	\caption{Mask layout for NGC253 Field B.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit53.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit54.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit55.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit56.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit57.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit58.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit59.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit60.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldB_Slits/NGC253_FieldB_Slit61.pdf}& 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for NGC253 Field B.}
\end{figure}


\clearpage
\subsection{NGC253 Field C}
\vfill
\begin{figure*}[h!]
	\center
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_NGC253_FieldC.pdf}}
  	\caption{Mask layout for NGC253 Field C.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit53.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit54.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit55.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit56.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit57.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit58.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit59.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit60.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit61.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit62.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit63.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit64.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit65.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit66.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit67.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit68.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC253_FieldC_Slits/NGC253_FieldC_Slit69.pdf}& 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for NGC253 Field C.}
\end{figure}


\clearpage
\subsection{NGC300 Field A}
\vfill
\begin{figure*}[h!]
	\center
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_NGC300_FieldA.pdf}}
  	\caption{Mask layout for NGC300 Field A.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldA_Slits/NGC300_FieldA_Slit53.pdf}& 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for NGC300 Field A.}
\end{figure}


\clearpage
\subsection{NGC300 Field B}
\vfill
\begin{figure*}[h!]
	\center
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_NGC300_FieldB.pdf}}
  	\caption{Mask layout for NGC300 Field B.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit53.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit54.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit55.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit56.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit57.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit58.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit59.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit60.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit61.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit62.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit63.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldB_Slits/NGC300_FieldB_Slit64.pdf}& 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for NGC300 Field B.}
\end{figure}


\clearpage
\subsection{NGC300 Field C}
\vfill
\begin{figure*}[h!]
	\center
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_NGC300_FieldC.pdf}}
  	\caption{Mask layout for NGC300 Field C.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit53.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit54.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit55.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit56.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit57.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit58.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit59.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit60.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit61.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit62.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit63.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit64.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldC_Slits/NGC300_FieldC_Slit65.pdf}& 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for NGC300 Field C.}
\end{figure}


\clearpage
\subsection{NGC300 Field D}
\vfill
\begin{figure*}[h!]
	\center
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_NGC300_FieldD.pdf}}
  	\caption{Mask layout for NGC300 Field D.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit53.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit54.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit55.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit56.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit57.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit58.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit59.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC300_FieldD_Slits/NGC300_FieldD_Slit60.pdf}& 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for NGC300 Field D.}
\end{figure}


\clearpage
\subsection{NGC7793 Field A}
\vfill
\begin{figure*}[h!]
	\center
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_NGC7793_FieldA.pdf}}
  	\caption{Mask layout for NGC7793 Field A.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit53.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit54.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit55.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit56.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit57.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit58.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit59.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit60.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit61.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit62.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit63.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/NGC7793_FieldA_Slits/NGC7793_FieldA_Slit64.pdf}& 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for NGC7793 Field A.}
\end{figure}


\clearpage


\subsection{Sextans A Field A}

\vfill
\begin{figure*}[h!]
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_SextansA_FieldA.pdf}}
  	\caption{Mask layout for Sextans A Field A.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/SextansA_FieldA_Slits/SextansA_FieldA_Slit23.pdf}& 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for Sextans Field A.}
\end{figure}




\clearpage



\subsection{WLM Field A}
\vfill
\begin{figure*}[h!]
	\center
   	\resizebox{1.0\hsize}{!}{\includegraphics{Figures/Masks/mask_WLM_FieldA.pdf}}
  	\caption{Mask layout for WLM Field A.}
\end{figure*}
\vfill

\begin{longtable}{cccc}
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit7.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit8.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit9.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit10.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit11.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit12.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit13.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit14.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit15.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit16.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit17.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit18.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit19.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit20.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit21.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit22.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit23.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit24.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit25.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit26.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit27.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit28.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit29.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit30.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit31.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit32.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit33.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit34.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit35.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit36.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit37.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit38.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit39.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit40.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit41.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit42.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit43.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit44.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit45.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit46.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit47.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit48.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit49.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit50.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit51.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit52.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit53.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit54.pdf}\\ 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit55.pdf}& 
\includegraphics[width=0.2\textwidth]{Figures/Masks/WLM_FieldA_Slits/WLM_FieldA_Slit56.pdf}& 
\end{longtable}

\vspace{-0.5cm}
\begin{figure}[h!]
  	\caption{Slit locations for WLM Field A.}
\end{figure}

